Multi-Level Multi-Fidelity Methods for Path Integral and Safe Control

Sampling-based approaches are widely used in systems without analytic models to estimate risk or find optimal control. However, gathering sufficient data in such scenarios can be prohibitively costly. On the other hand, in many situations, low-fidelity models or simulators are available from which samples can be obtained at low cost. In this paper, we propose an efficient approach for risk quantification and path integral control that leverages such data from multiple models with heterogeneous sampling costs. A key technical novelty of our approach is the integration of Multi-level Monte Carlo (MLMC) and Multi-fidelity Monte Carlo (MFMC) that enable data from different time and state representations (system models) to be jointly used to reduce variance and improve sampling efficiency. We also provide theoretical analysis of the proposed method and show that our estimator is unbiased and consistent under mild conditions. Finally, we demonstrate via numerical simulation that the proposed method has improved computation (sampling costs) vs. accuracy trade-offs for risk quantification and path integral control.

==> MACPdef-ams.tex <==
% Definitions that require the amsmath.sty and amsthm.sty files
% Time-stamp: <13/05/12 17:29:30 mcarreira-perpinan>

% -------------- Operators --------------

% Probability
\newcommand{\Eop}{\operatorname{E}}
\newcommand{\mean}[2][]{\ensuremath{\Eop_{#1}\left\{#2\right\}}}
\newcommand{\meanop}{\operatorname{mean}}
\newcommand{\Mean}[2][]{\ensuremath{\meanop_{#1}\left\{#2\right\}}}
\newcommand{\aveop}{\Eop}
% \newcommand{\ave}[2][]{\ensuremath{\aveop_{#1}\left\{#2\right\}}}
% \newcommand{\varop}{\operatorname{var}}
% \newcommand{\var}[2][]{\ensuremath{\varop_{#1}\left\{#2\right\}}}
% \newcommand{\stdevop}{\operatorname{stdev}}
\newcommand{\stdev}[2][]{\ensuremath{\stdevop_{#1}\left\{#2\right\}}}
\newcommand{\covop}{\operatorname{cov}}
\newcommand{\cov}[2][]{\ensuremath{\covop_{#1}\left\{#2\right\}}}
\newcommand{\eff}{\operatorname{eff}}
\newcommand{\Prop}{\operatorname{Pr}}
\newcommand{\prob}[1]{\ensuremath{\Prop\left[#1\right]}}
\newcommand{\Volume}{\operatorname{vol}}
\newcommand{\volume}[1]{\ensuremath{\Volume\left(#1\right)}}
\newcommand{\Domain}{\operatorname{dom}}
\newcommand{\dom}[1]{\ensuremath{\Domain\left(#1\right)}}

% Functions
\newcommand{\erf}{\operatorname{erf}}
\newcommand{\sgnop}{\operatorname{sgn}}
\newcommand{\sgn}[1]{\ensuremath{\sgnop\left(#1\right)}}

% Information theory
\newcommand{\KLop}{\operatorname{D}}
%\newcommand{\KLop}{\operatorname{KL}}
\newcommand{\KL}[2]{\KLop\left(#1\lVert#2\right)} % Kullback-Leibler divergence
\newcommand{\KLsym}[2]{\KLop\left(#1,#2\right)}   % Symmetrised KL divergence

% Set theory
% Are "card" and "im" the correct names in English?
\newcommand{\cardop}{\operatorname{card}}
\newcommand{\card}[1]{\ensuremath{\cardop\left(#1\right)}}
\newcommand{\im}{\operatorname{im}}
\newcommand{\vol}{\operatorname{vol}}
\newcommand{\convop}{\operatorname{conv}}
\newcommand{\conv}[1]{\ensuremath{\convop\left(#1\right)}}

% Matrices
\newcommand{\diagop}{\operatorname{diag}}
\newcommand{\diag}[1]{\ensuremath{\diagop\left(#1\right)}}
\newcommand{\cof}{\operatorname{cof}}           % Cofactor of a matrix element
\newcommand{\adj}{\operatorname{adj}}           % Adjunt matrix
\newcommand{\traceop}{\operatorname{tr}}
\newcommand{\trace}[1]{\ensuremath{\traceop\left(#1\right)}}
\newcommand{\rankop}{\operatorname{rank}}
\newcommand{\rank}[1]{\ensuremath{\rankop\left(#1\right)}}
\newcommand{\Nullop}{\operatorname{null}}
\newcommand{\Null}[1]{\ensuremath{\Nullop\left(#1\right)}}
\newcommand{\rangeop}{\operatorname{range}}
\newcommand{\range}[1]{\ensuremath{\rangeop\left(#1\right)}}
\newcommand{\Dimop}{\operatorname{dim}}
\newcommand{\Dim}[1]{\ensuremath{\Dimop\left(#1\right)}}
\newcommand{\spanop}{\operatorname{span}}
\newcommand{\spn}[1]{\ensuremath{\spanop\left\{#1\right\}}}
\newcommand{\vectop}{\operatorname{vec}}
\newcommand{\vect}[1]{\ensuremath{\vectop\left(#1\right)}}
\newcommand{\condop}{\operatorname{cond}}
\newcommand{\cond}[1]{\ensuremath{\condop\left(#1\right)}}

% -------------- Theorem environments --------------
\let\proof\relax
\let\endproof\relax
\let\example\relax
\let\endexample\relax
\usepackage{amsthm}

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{assumption}{Assumption}
\newtheorem{preliminary}{Preliminary}
 %\theoremstyle{plain}
\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{condition}{Condition}
\newtheorem{example}{Example}
\theoremstyle{plain}% default
\newtheorem{thm}{Theorem}[section]

\theoremstyle{remark}
\newtheorem{remark}{Remark}

% % \newtheorem{lemma}[thm]{Lemma}
% \newtheorem*{lemma*}{Lemma}
% \newtheorem{prop}[thm]{Proposition}
% \newtheorem*{prop*}{Proposition}
% \newtheorem{cor}[thm]{Corollary}
% \newtheorem{obs}[thm]{Observation}

% \theoremstyle{definition}
% \newtheorem{defn}{Definition}[section]
% \newtheorem*{defn*}{Definition}
% \newtheorem{exmp}{Example}[section]
% \newtheorem*{exmp*}{Example}
% \newtheorem{conj}{Conjecture}[section]
% \newtheorem*{conj*}{Conjecture}

% \theoremstyle{remark}
% \newtheorem{rmk}[thm]{Remark}
% \newtheorem*{rmk*}{Remark}
% \newcommand{\ubar}[1]{\text{\b{$#1$}}}

%%% Local Variables: 
%%% mode: plain-tex
%%% TeX-master: t
%%% End: 


==> MACPdef.tex <==
% Miguel A. Carreira-Perpinan's LaTeX macros.
% Time-stamp: <13/05/30 14:02:52 mcarreira-perpinan>

% Definitions that require only standard LaTeX2e things

% Letters used for matrices and vectors (boldface), for functions (roman), etc.
\newcommand{\mA}{\ensuremath{\mathbf{A}}}
\newcommand{\mB}{\ensuremath{\mathbf{B}}}
\newcommand{\mC}{\ensuremath{\mathbf{C}}}
\newcommand{\mD}{\ensuremath{\mathbf{D}}}
\newcommand{\mE}{\ensuremath{\mathbb{E}}}
\newcommand{\mF}{\ensuremath{\mathbf{F}}}
\newcommand{\mG}{\ensuremath{\mathbf{G}}}
\newcommand{\mH}{\ensuremath{\mathbf{H}}}
\newcommand{\mI}{\ensuremath{\mathbf{I}}}
\newcommand{\mJ}{\ensuremath{\mathbf{J}}}
\newcommand{\mK}{\ensuremath{\mathbf{K}}}
\newcommand{\mL}{\ensuremath{\mathbf{L}}}
\newcommand{\mM}{\ensuremath{\mathbf{M}}}
\newcommand{\mN}{\ensuremath{\mathbf{N}}}
\newcommand{\mO}{\ensuremath{\mathbf{O}}}
\newcommand{\mP}{\ensuremath{\mathbb{P}}}
\newcommand{\mQ}{\ensuremath{\mathbf{Q}}}
%\newcommand{\R}{\ensuremath{\mathbf{R}}} % PROSPER defines \R
\newcommand{\mR}{\ensuremath{\mathbf{R}}}
\newcommand{\mS}{\ensuremath{\mathbf{S}}}
\newcommand{\mT}{\ensuremath{\mathbf{T}}}
\newcommand{\mU}{\ensuremath{\mathbf{U}}}
\newcommand{\mV}{\ensuremath{\mathbf{V}}}
\newcommand{\mW}{\ensuremath{\mathbf{W}}}
\newcommand{\mX}{\ensuremath{\mathbf{X}}}
\newcommand{\mY}{\ensuremath{\mathbf{Y}}}
\newcommand{\mZ}{\ensuremath{\mathbf{Z}}}
\newcommand{\va}{\ensuremath{\mathbf{a}}}
\newcommand{\vb}{\ensuremath{\mathbf{b}}}
\newcommand{\vc}{\ensuremath{\mathbf{c}}}
\newcommand{\vd}{\ensuremath{\mathbf{d}}}
\newcommand{\ve}{\ensuremath{\mathbf{e}}}
\newcommand{\vf}{\ensuremath{\mathbf{f}}}
\newcommand{\vg}{\ensuremath{\mathbf{g}}}
\newcommand{\vh}{\ensuremath{\mathbf{h}}}
\newcommand{\vk}{\ensuremath{\mathbf{k}}}
\newcommand{\vl}{\ensuremath{\mathbf{l}}}
\newcommand{\vell}{\ensuremath{\mathbf{\ell}}}
\newcommand{\vm}{\ensuremath{\mathbf{m}}}
\newcommand{\vn}{\ensuremath{\mathbf{n}}}
\newcommand{\vp}{\ensuremath{\mathbf{p}}}
\newcommand{\vq}{\ensuremath{\mathbf{q}}}
\newcommand{\vr}{\ensuremath{\mathbf{r}}}
\newcommand{\vs}{\ensuremath{\mathbf{s}}}  % TIPA defines \s and LaTeX \ss!
\newcommand{\vt}{\ensuremath{\mathbf{t}}}
\newcommand{\vu}{\ensuremath{\mathbf{u}}}
\newcommand{\vv}{\ensuremath{\mathbf{v}}}
%\renewcommand{\v}{\ensuremath{\mathbf{v}}}
\newcommand{\vw}{\ensuremath{\mathbf{w}}}
\newcommand{\vx}{\ensuremath{\mathbf{x}}}
\newcommand{\vy}{\ensuremath{\mathbf{y}}}
\newcommand{\vz}{\ensuremath{\mathbf{z}}}
\newcommand{\0}{\ensuremath{\mathbf{0}}}
\newcommand{\1}{\ensuremath{\mathbf{1}}}

% Bold symbols and greek letters
\newcommand{\balpha}{\ensuremath{\boldsymbol{\alpha}}}
\newcommand{\bbeta}{\ensuremath{\boldsymbol{\beta}}}
\newcommand{\bdelta}{\ensuremath{\boldsymbol{\delta}}}
\newcommand{\bepsilon}{\ensuremath{\boldsymbol{\epsilon}}}
\newcommand{\binfty}{\ensuremath{\boldsymbol{\infty}}}
\newcommand{\bkappa}{\ensuremath{\boldsymbol{\kappa}}}
\newcommand{\blambda}{\ensuremath{\boldsymbol{\lambda}}}
\newcommand{\bmu}{\ensuremath{\boldsymbol{\mu}}}
\newcommand{\bnu}{\ensuremath{\boldsymbol{\nu}}}
\newcommand{\bphi}{\ensuremath{\boldsymbol{\phi}}}
\newcommand{\bpi}{\ensuremath{\boldsymbol{\pi}}}
\newcommand{\bpsi}{\ensuremath{\boldsymbol{\psi}}}
\newcommand{\brho}{\ensuremath{\boldsymbol{\rho}}}
\newcommand{\bsigma}{\ensuremath{\boldsymbol{\sigma}}}
\newcommand{\btau}{\ensuremath{\boldsymbol{\tau}}}
\newcommand{\btheta}{\ensuremath{\boldsymbol{\theta}}}
\newcommand{\bxi}{\ensuremath{\boldsymbol{\xi}}}
\newcommand{\bzeta}{\ensuremath{\boldsymbol{\zeta}}}

\newcommand{\bDelta}{\ensuremath{\boldsymbol{\Delta}}}
\newcommand{\bGamma}{\ensuremath{\boldsymbol{\Gamma}}}
\newcommand{\bLambda}{\ensuremath{\boldsymbol{\Lambda}}}
\newcommand{\bPhi}{\ensuremath{\boldsymbol{\Phi}}}
\newcommand{\bPi}{\ensuremath{\boldsymbol{\Pi}}}
\newcommand{\bPsi}{\ensuremath{\boldsymbol{\Psi}}}
\newcommand{\bSigma}{\ensuremath{\boldsymbol{\Sigma}}}
\newcommand{\bTheta}{\ensuremath{\boldsymbol{\Theta}}}
\newcommand{\bXi}{\ensuremath{\boldsymbol{\Xi}}}
\newcommand{\bUpsilon}{\ensuremath{\boldsymbol{\Upsilon}}}

% Blackboard bold
\newcommand{\bbC}{\ensuremath{\mathbb{C}}}
\newcommand{\bbH}{\ensuremath{\mathbb{H}}}
\newcommand{\bbN}{\ensuremath{\mathbb{N}}}
\newcommand{\bbR}{\ensuremath{\mathbb{R}}}
\newcommand{\bbS}{\ensuremath{\mathbb{S}}}
\newcommand{\bbZ}{\ensuremath{\mathbb{Z}}}
\newcommand{\bbE}{\ensuremath{\mathbb{E}}}
% Graph
\newcommand\gA{{\mathcal{A}}}
\newcommand\gB{{\mathcal{B}}}
\newcommand\gC{{\mathcal{C}}}
\newcommand\gD{{\mathcal{D}}}
\newcommand\gE{{\mathcal{E}}}
\newcommand\gF{{\mathcal{F}}}
\newcommand\gG{{\mathcal{G}}}
\newcommand\gH{{\mathcal{H}}}
\newcommand\gI{{\mathcal{I}}}
\newcommand\gJ{{\mathcal{J}}}
\newcommand\gK{{\mathcal{K}}}
\newcommand\gL{{\mathcal{L}}}
\newcommand\gM{{\mathcal{M}}}
\newcommand\gN{{\mathcal{N}}}
\newcommand\gO{{\mathcal{O}}}
\newcommand\gP{{\mathcal{P}}}
\newcommand\gQ{{\mathcal{Q}}}
\newcommand\gR{{\mathcal{R}}}
\newcommand\gS{{\mathcal{S}}}
\newcommand\gT{{\mathcal{T}}}
\newcommand\gU{{\mathcal{U}}}
\newcommand\gV{{\mathcal{V}}}
\newcommand\gW{{\mathcal{W}}}
\newcommand\gX{{\mathcal{X}}}
\newcommand\gY{{\mathcal{Y}}}
\newcommand\gZ{{\mathcal{Z}}}

% Relational operators
% \bydef puts ``def'' over the equals sign and means ``is by definition
% equal to''. Another possibility is to use the \triangleq symbol.
\newcommand{\bydef}{\stackrel{\mathrm{\scriptscriptstyle def}}{=}}
% \simbydef puts ``def'' over the ~ sign and means ``is by definition
% distributed as''.
\newcommand{\simbydef}{\stackrel{\mathrm{\scriptscriptstyle def}}{\sim}}
\newcommand{\proptobydef}{\stackrel{\mathrm{\scriptscriptstyle def}}{\propto}}

% Other functions
\newcommand{\abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\ceil}[1]{\lceil#1\rceil}
\newcommand{\floor}[1]{\lfloor#1\rfloor}

% Left superscript
% (from http://www.maths.univ-rennes1.fr/~edix/sgahtml/typesetting_rules.html)
\newcommand{\leftexp}[2]{{\vphantom{#2}}^{#1}{#2}}

% Box of text (for pictures, tables, etc.), without frames. Arguments:
%   #1: separation between rows of text as a multiple of LaTeX's default
%       (optional, default 1).
%   #2: position (one of t, b, c).
%   #3: format (one of l, r, c or even p{2cm}).
%   #4: text, which can include line breaks (\\).
\newcommand{\caja}[4][1]{{%
    \renewcommand{\arraystretch}{#1}%
    \begin{tabular}[#2]{@{}#3@{}}%
      #4%
    \end{tabular}%
    }}

% The amsart class has its own \keywords command, in which case we
% don't replace it.
\providecommand{\keywords}[1]{\vspace*{0.5\baselineskip}\par\noindent\textbf{Keywords:} #1}

% The logos (AmSLaTeX, BibTeX, etc.) are defined in texnames.sty.

% List environments
%
% "simplelist": useful for compact lists. Use it instead of "itemize".
% Optional argument: the bullet (default \triangleright). Other nice
% bullets are available in the Zapf Dingbats font (e.g. \ding{166} in
% the pifont package).
%
\newenvironment{simplelist}[1][$\triangleright$]%
{%
\begin{list}{#1}{
\vspace{-\topsep}
\vspace{-\partopsep}
\setlength{\itemindent}{0cm}
\setlength{\rightmargin}{0cm}
\setlength{\listparindent}{0cm}
\settowidth{\labelwidth}{#1}
\setlength{\leftmargin}{\labelwidth}
\addtolength{\leftmargin}{\labelsep}
\setlength{\itemsep}{0cm}
%\setlength{\leftmargin}{0cm}
%\setlength{\labelwidth}{0cm}
}%
}%
{%
\end{list}
\vspace{-\topsep}
\vspace{-\partopsep}
}

%
% enumthm: an enumerated list intended to appear in theorems and not
% to be nested. Each item is numbered in Roman numerals in parentheses.
% A suitable way to refer to an item is:
% Theorem~\ref{thm:pithagoras}(\ref{en:triangle}) states...
\newenvironment{enumthm}%
{\begin{enumerate}%
\renewcommand{\theenumi}{\roman{enumi}}%
\renewcommand{\labelenumi}{(\theenumi)}}%
{\end{enumerate}}

% Commands for the hyperref package (they also require the url package).
% In all cases the typesetting style is tt by default but can be changed
% with the \urlstyle command, e.g. \urlstyle{tt}.
%
% \MACPhref[text]{link} typesets text (default = link) in tt and
% hyperlinks to link, e.g. \MACPhref{http://www.dcs.shef.ac.uk/~miguel}.
\newcommand{\MACPhref}[2][\DefaultOpt]{\def\DefaultOpt{#2}%
  \href{#2}{\url{#1}}}
%
% \MACPmailto[text]{email} typesets text (default = email) in tt and
% hyperlinks to email as mailto:email, e.g. \MACPmailto{miguel@dcs.shef.ac.uk}.
\newcommand{\MACPmailto}[2][\DefaultOpt]{\def\DefaultOpt{#2}%
  \href{mailto:#2}{\url{#1}}}

% % Hyphenation
% \hyphenation{elec-tro-pa-la-tog-ra-phy}

% % From the amsbook.cls file version 2.04
% \hyphenation{acad-e-my acad-e-mies af-ter-thought anom-aly anom-alies
% an-ti-deriv-a-tive an-tin-o-my an-tin-o-mies apoth-e-o-ses
% apoth-e-o-sis ap-pen-dix ar-che-typ-al as-sign-a-ble as-sist-ant-ship
% as-ymp-tot-ic asyn-chro-nous at-trib-uted at-trib-ut-able bank-rupt
% bank-rupt-cy bi-dif-fer-en-tial blue-print busier busiest
% cat-a-stroph-ic cat-a-stroph-i-cally con-gress cross-hatched data-base
% de-fin-i-tive de-riv-a-tive dis-trib-ute dri-ver dri-vers eco-nom-ics
% econ-o-mist elit-ist equi-vari-ant ex-quis-ite ex-tra-or-di-nary
% flow-chart for-mi-da-ble forth-right friv-o-lous ge-o-des-ic
% ge-o-det-ic geo-met-ric griev-ance griev-ous griev-ous-ly
% hexa-dec-i-mal ho-lo-no-my ho-mo-thetic ideals idio-syn-crasy
% in-fin-ite-ly in-fin-i-tes-i-mal ir-rev-o-ca-ble key-stroke
% lam-en-ta-ble light-weight mal-a-prop-ism man-u-script mar-gin-al
% meta-bol-ic me-tab-o-lism meta-lan-guage me-trop-o-lis
% met-ro-pol-i-tan mi-nut-est mol-e-cule mono-chrome mono-pole
% mo-nop-oly mono-spline mo-not-o-nous mul-ti-fac-eted mul-ti-plic-able
% non-euclid-ean non-iso-mor-phic non-smooth par-a-digm par-a-bol-ic
% pa-rab-o-loid pa-ram-e-trize para-mount pen-ta-gon phe-nom-e-non
% post-script pre-am-ble pro-ce-dur-al pro-hib-i-tive pro-hib-i-tive-ly
% pseu-do-dif-fer-en-tial pseu-do-fi-nite pseu-do-nym qua-drat-ic
% quad-ra-ture qua-si-smooth qua-si-sta-tion-ary qua-si-tri-an-gu-lar
% quin-tes-sence quin-tes-sen-tial re-arrange-ment rec-tan-gle
% ret-ri-bu-tion retro-fit retro-fit-ted right-eous right-eous-ness
% ro-bot ro-bot-ics sched-ul-ing se-mes-ter semi-def-i-nite
% semi-ho-mo-thet-ic set-up se-vere-ly side-step sov-er-eign spe-cious
% spher-oid spher-oid-al star-tling star-tling-ly sta-tis-tics
% sto-chas-tic straight-est strange-ness strat-a-gem strong-hold
% sum-ma-ble symp-to-matic syn-chro-nous topo-graph-i-cal tra-vers-a-ble
% tra-ver-sal tra-ver-sals treach-ery turn-around un-at-tached
% un-err-ing-ly white-space wide-spread wing-spread wretch-ed
% wretch-ed-ly Eng-lish Euler-ian Feb-ru-ary Gauss-ian
% Hamil-ton-ian Her-mit-ian Jan-u-ary Japan-ese Kor-te-weg
% Le-gendre Mar-kov-ian Noe-ther-ian No-vem-ber Rie-mann-ian Sep-tem-ber}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 

